Semantic Analysis of Macro Usage for Portability

C is an unsafe language. Researchers have been developing tools to port C to safer languages such as Rust, Checked C, or Go. Existing tools, however, resort to preprocessing the source file first, then porting the resulting code, leaving barely recognizable code that loses macro abstractions. To preserve macro usage, porting tools need analyses that understand macro behavior to port to equivalent constructs. But macro semantics differ from typical functions, precluding simple syntactic transformations to port them. We introduce the first comprehensive framework for analyzing the portability of macro usage. We decompose macro behavior into 26 fine-grained properties and implement a program analysis tool, called Maki, that identifies them in real-world code with 94% accuracy. We apply Maki to 21 programs containing a total of 86,199 macro definitions. We found that real-world macros are much more portable than previously known. More than a third (37%) are easy-to-port, and Maki provides hints for porting more complicated macros. We find, on average, 2x more easy-to-port macros and up to 7x more in the best case compared to prior work. Guided by Maki's output, we found and hand-ported macros in four real-world programs. We submitted patches to Linux maintainers that transform eleven macros, nine of which have been accepted.

==> Makefile <==
# ----------------------------------------------------------------------------
#                         Simple latex makefile
#
#                  Original author: Robert Grimm, rgrimm@cs.nyu.edu
#                  Updated: Paul Gazzillo, paul.gazzillo@ucf.edu
# ----------------------------------------------------------------------------

# ----------------------------------------------------------------------------
#  Tools
# ----------------------------------------------------------------------------

PDFLATEX     = pdflatex
BIBTEX       = bibtex
MV           = mv
RM           = rm -f

# ----------------------------------------------------------------------------
#  Source file(s)
# ----------------------------------------------------------------------------

SOURCE       = \
	main.tex

# ----------------------------------------------------------------------------
#  Figures
# ----------------------------------------------------------------------------

FIGURES      = 


# ----------------------------------------------------------------------------
#  Bibliography
# ----------------------------------------------------------------------------

BIBLIOGRAPHY = references.bib

# ----------------------------------------------------------------------------
#  Rules
# ----------------------------------------------------------------------------

AUX_FILES = $(SOURCE:%.tex=%.aux)
BBL_FILES = $(SOURCE:%.tex=%.bbl)
BLG_FILES = $(SOURCE:%.tex=%.blg)
DVI_FILES = $(SOURCE:%.tex=%.dvi)
LOG_FILES = $(SOURCE:%.tex=%.log)
OUT_FILES = $(SOURCE:%.tex=%.out)
PDF_FILES = $(SOURCE:%.tex=%.pdf)
FLG_FILES = $(SOURCE:%.tex=%.4LG)
BAK_FILES = $(SOURCE:%.tex=%.BAK)
WRD_FILES = $(SOURCE:%.tex=%.WRD)

.PHONY: all clean publish
.SECONDARY: $(BBL_FILES)

all : $(PDF_FILES)

%.pdf : %.tex $(wildcard *.tex) %.bbl $(FIGURES)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl : %.tex $(wildcard *.tex) $(BIBLIOGRAPHY)
	$(PDFLATEX) $<
	-$(BIBTEX) $*
	$(PDFLATEX) $<

clean :
	$(RM) $(AUX_FILES)
	$(RM) $(BBL_FILES)
	$(RM) $(BLG_FILES)
	$(RM) $(DVI_FILES)
	$(RM) $(LOG_FILES)
	$(RM) $(OUT_FILES)
	$(RM) $(PDF_FILES)
	$(RM) $(FLG_FILES)
	$(RM) $(BAK_FILES)
	$(RM) $(WRD_FILES)


==> background.tex <==
Let us look more closely at the syntax and semantics of function macros.
In this section, we describe \emph{aligned} macros, i.e., those that follow C syntax, and prior work on identifying aligned macros.
Then we illustrate the differences between macro and C functions and how those differences affect the viability of transformation.

\subsection{Aligned Macros}
\label{subsec:alignment}

The C preprocessor is a \emph{lexical} preprocessor~\cite{cppmanual}, i.e., it operates at the token-level of the source file.
Therefore, preprocessor macro definitions are sequences of C tokens and have no regard for the syntax of C, which is why macros like the \texttt{vmcase} macro are legal.
While much prior work has looked at the interaction between lexical preprocessing and C syntax~\cite{superc,typechef,dietrich,crefactory,yacfe,mapr}, Cpp2C only needs to identify what macros are aligned, otherwise the macro is not a candidate for transformation.

Finding aligned macros entails preprocessing and parsing the original source and checking whether a preprocessed macro's expansion corresponds one-to-one with a subtree of the abstract syntax tree (AST).
Prior work already exists to map preprocessed source back to the unpreprocessed source (clang's parser~\cite{clang}) as well as to track macro expansion alignment with the C AST (the cppsig plugin to clang~\cite{dietrich}).
Cpp2C leverages both of these technologies to find aligned macros.
The latter work, CPPSIG, also records the types of macro parameters, which \tool uses in the transformation to infer the types of the C function.










\begin{figure}
\begin{subfigure}{.54\columnwidth}
\begin{lstlisting}[style=CStyle]
#define FOO() 1 + 2
FOO();
0 * FOO() * 3;
\end{lstlisting}
\caption{\texttt{FOO} before preprocessing.}
\label{fig:wellformed:foo:before}
\end{subfigure}
\begin{subfigure}{.45\columnwidth}
\begin{lstlisting}[style=CStyle]
/* empty line */
1 + 2
0 * 1 + 2 * 3
\end{lstlisting}
\caption{\texttt{FOO} after preprocessing.}
\label{fig:wellformed:foo:after}
\end{subfigure}
\caption{Examples of aligned and unaligned macro expansions.}
\label{fig:wellformed}
\end{figure}

We illustrate alignment with a simple macro in Figure~\ref{fig:wellformed:foo:before}.
\verb'FOO()' expands to the tokens \verb'1 + 2' (Figure~\ref{fig:wellformed:foo:after}), which on its face appears to be aligned since it lines up exactly with a C arithmetic expression subtree, i.e., \red{(+ (1 2))}.
Indeed, the expansion of \verb'FOO();' becomes a valid C expression statement (line~2) that evaluates to \verb'3'.

If \verb'FOO' were a C function, the expression would be equivalent to \verb'0 * (1 + 2) * 3' and evaluate to \verb'0', since the function value would be computed before it is used in the expression.
But \verb'FOO' is a macro: when it is expanded on line~3, the tokens \verb'0 * FOO() * 3' become \verb'0 * 1 + 2 * 3', which evaluates to \verb'6', because of C's order of operations.
This phenomenon, called operator misnesting, is a well-known pitfall of the preprocessor~\cite{cppmanual}. and it is possible because the preprocessor is lexical, enforcing no syntax rules.
The \verb'FOO' example shows that we cannot look only at a macro's definition, but that our transformation \emph{must take into account both the definition and all of its expansion simultaneously to determine equivalence}.







\pg{how to find the types?  polymorphism.  why only expressions?}


==> macros-vs-functions.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c}
         \textbf{Macros} & \textbf{Functions} \\ \hline
         Dynamically-scoped & Lexically-scoped \\ \hline
         Untyped & Statically typed \\ \hline
         Call-by-name & Call-by-value \\ \hline
         Can manipulate tokens & Cannot manipulate tokens \\
    \end{tabular}
    \caption{Differences between macro invocations and function calls.}
    \label{tab:macros-vs-functions}
\end{table}
\brent{We classify each property as belonging to at least one of four categories of differences between macro invocations and function calls listed in Table~\ref{tab:macros-vs-functions}: differences in scoping rules, typing rules, calling convention, and token-manipulation ability.
We have chosen these specific categories because they encompass all semantic differences between macros and functions.}


==> transformations.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{ll}
        \textbf{Portability level} & \textbf{Code changes} \\
        \hline
        No changes & None \\
        Definition-adapting & Alter macro definition \\
        Calling-convention-adapting & Alter macro arguments \\
        Scope-adapting & \makecell[l]{Rename and/or reorder \\ of existing declarations} \\
        Thunkizing & Create thunks \\
        Callsite-context-altering & \makecell[l]{Alter the invocation's \\ surrounding AST context} \\
        Metaprogramming & Use metaprogramming tools \\
    \end{tabular}
    \caption{Code change portability levels.}
    \label{tab:transformations}
\end{table}

In this section we present a series of portability levels for measuring how well code changes help porting tools preserve macro abstractions.
Intuitively, a highly portable code change enables a porting tool to translate a macro to code in the target language that looks more similar to the original macro than a lesser portable code change would.
Table~\ref{sec:transformations} lists the 7 portability levels, each described by the code changes they require.
A transformation in the first level entails code changes that do not at all help porting tools preserve macro abstractions, while a transformation in the final level only entails code changes that best help porting tools preserve macro abstractions.
In Section~\ref{sec:evaluation}, we apply these levels to gauge the amount of manual effort necessary to port macros in real programs.

The lowest portability level is for when \textit{no changes} are made to a macro invocation, and instead leave it for the CPP to expand during preprocessing.
Not changing macro invocations does not help porting tools preserve them, because preprocessing macro invocations removes all traces of them from their original programs.
Unfortunately, modern porting tools do preprocess macro invocations, because they can only parse C code, not CPP code; and the simplest way to remove CPP code from a program is to preprocess it.

The next portability level contains \textbf{metaprogramming} code changes.
Metaprogramming code changes require developers to create or use new metaprogramming tools to achieve the same effect as the original code.
These code changes are necessary, for instance, for macro invocations which use stringification or token-pasting, since these operations are exclusive to the CPP and have no C analogue.
For example, consider the invocation of the macro \verb|DECLARE_STRING| from \gv~\cite{gv-3.7.4}:
\begin{lstlisting}[style=CStyle]
#  define DECLARE_STRING(aaa) \
      extern char * s_ ## aaa;
DECLARE_STRING(medias)|\label{line:invoke-declare-string}|
\end{lstlisting}
The invocation of \verb|DECLARE_STRING| on line~\ref{line:invoke-declare-string} expands to the declaration \verb|extern char * s_medias;|.
The declaration's qualifier (\verb|extern|), type (\verb|char *|), and ending semicolon come from the definition of \verb|DECLARE_STRING|.
The invocation creates the name of the declaration, \verb|s_medias|, by using the token-pasting operator (\verb|##|) to concatenate the token \verb|s_| with the tokens passed to the \verb|aaa| argument.
There is no built-in C language construct that can concatenate tokens together like this, so the only way to achieve this in C would be to modify the program to use some other metaprogramming tool that can concatenate tokens together to form variable declarations.
Because metaprogramming code changes can significantly alter a program, we anticipate that developers will hardly, if ever, use them to improve macro portability.

After metaprogramming code changes we have \textbf{thunkizing} code changes.
As their name suggests, thunkizing code changes involve the creation of thunks, another name for functions used to delay computation until a later point.
These thunks are used to address differences in calling conventions between macro invocations and function calls.
Function calls follow a call-by-value calling convention, and as such evaluate their arguments eagerly; whereas macro invocations use a call-by-name evaluation strategy, and evaluate their arguments each time they are needed.
By replacing certain arguments with thunks and calling them wherever they are used, function calls can simulate call-by-name evaluation.
As an example, here is the macro \verb|MEM_SAME| defined in \rcs~\cite{rcs-5.10.0}:
\begin{lstlisting}[style=CStyle]
#define MEM_SAME(n,a,b)  (0 == memcmp ((a), (b), (n)))
char const *x, *p, *nz;
size_t nl, xl;
if (xl <= nl && MEM_SAME (xl, (p = nz - xl), x))|\label{line:invoke-mem-same}|
\end{lstlisting}
On line~\ref{line:invoke-mem-same}, the second argument to the invocation \verb|MEM_SAME| is the side-effecting expression \verb|(p = nz - xl)|.
Because macro invocation arguments are evaluated lazily, these side-effects are not evaluated when the macro is invoked, but at the appropriate point in the expanded code.
This is unlike functions, which evaluate their arguments eagerly.
Admittedly, whether arguments are evaluated eagerly or lazily does not matter for the above example.
However, if we truly wanted to emulate the lazy evaluation of macro invocations with function calls, we could do so by turning the argument with side-effects into a thunk, and then calling that thunk wherever we originally expanded the argument.
For instance, we can use a thunkizing code change to turn the invocation of \verb|MEM_SAME| on line~\ref{line:invoke-mem-same} into a portable function call as follows:
\vspace{0.5em}
\begin{lstlisting}[style=CStyle]
char const *foo(char const **p, char const *nz, size_t xl) {
    return ((*p) = nz - xl);
}
bool MEM_SAME(size_t n, char const *(*a)(char const **, char const *, size_t),
                            char const *b, char const **p, char const *nz, size_t xl) {
    return (0 == memcmp (((*a)(p, nz, xl)), (b), (n)));|\label{line:call-foo}|
}
char const *x, *p, *nz;
size_t nl, xl;
if (xl <= nl && MEM_SAME (xl, foo, x, &p, nz, xl))|\label{line:call-mem-same}|
\end{lstlisting}

In the above code, \verb|MEM_SAME|'s second argument \verb|(p = nz - xl)| has been extracted into the function \verb|foo|.
We pass \verb|foo| to the call to \verb|MEM_SAME| on line~\ref{line:call-mem-same} and call \verb|foo| on line~\ref{line:call-foo}.
This ensures that \verb|MEM_SAME|'s second argument is not evaluated until it is called while evaluating the body of the transformed function definition of \verb|MEM_SAME|.

Although not as complex as metaprogramming code changes, thunkizing code changes are still tedious and often challenging to perform manually.
As such, we believe developers would be unlikely to use thunkizing code changes in production software.

The fourth level of the abstraction-preservation scale is for \textbf{callsite-context-altering} code changes.
These code changes modify the code directly surrounding macro invocations.
Callsite-context-altering code changes are chiefly used to make unaligned macro invocations more portable by turning macro invocations which do not expand to individual AST nodes into function calls, which are single AST nodes.
To turn an unaligned macro invocation into a function call, we need to change it and its arguments (if any) to completely comprise individual AST nodes, since C function calls and their arguments each comprise single AST nodes.
We can do this by moving some of the code surrounding the unaligned macro invocation into its definition before transforming it.
Great care must be taken when making this change to ensure that the resulting code is behaviorally equivalent to the first.
For instance, consider the following contrived example:
\begin{lstlisting}[style=CStyle]
#define ADD(a, b) a + b
5 * ADD(2, 3);|\label{line:invoke-add}|
\end{lstlisting}
The expanded form of line~\ref{line:invoke-add} is \verb|5 * 2 + 3|.
The subexpression \verb|2 + 3| comes from the expansion of \verb|ADD|, so one would think it would be evaluated first before being multiplied with \verb|5|.
However, because the CPP operates at a token-level, the entire expanded code is first parsed, and then evaluated.
So what really happens in that \verb|5 * 2| is evaluated first, and then this product is added to \verb|3|.
This is a common CPP pitfall~\cite{cppmanual-operator-precedence}, so the developer probably did not intend for this to happen.
If so, then we can change the above code as follows:
\begin{lstlisting}[style=CStyle]
int ADD(int a, int b) { return a + b; }
5 * ADD(2, 3);|\label{line:call-add}|
\end{lstlisting}
Now the call to \verb|ADD| on line~\ref{line:call-add} will be evaluated first, and the result will be multiplied with \verb|5|.
If the original code was correct, however, then we should instead change the original macro invocation like so:
\begin{lstlisting}[style=CStyle]
int ADD(int a, int b) { return a + b; }
ADD(5 * 2, 3);|\label{line:call-add-2}|
\end{lstlisting}
Now, the call to \verb|ADD| on line~\ref{line:call-add-2} evaluates it argument \verb|5 * 2| first before evaluating its body, so the original invocation's behavior is preserved.
These past two examples show that in order to correctly turn an unaligned invocation into C code, one needs a proper understanding of both the macro invocation's current and intended behavior.

The next level of the scale is reserved for \textbf{declaration-altering} code changes.
Declaration-altering code changes rename or rearrange a program's declarations.
Take, for example, the invocation of the macro \verb|nonlinear| defined in \gnuplot~\cite{gnuplot-5.4.4}:
\begin{lstlisting}[style=CStyle]
# define nonlinear(axis) ((axis)->linked_to_primary != NULL && (axis)->link_udf->at != NULL)
typedef struct axis { ... } AXIS;
AXIS *secondary;
if (nonlinear(secondary))
\end{lstlisting}
The macro \verb|nonlinear| accepts a single argument \verb|axis| of type \verb|AXIS *| as input, and returns true if \verb|axis| meets some conditions.
We can port \verb|nonlinear| by turning it into a function, but to do so we must first replace its macro definition with a function definition.
This is necessary to transform any macro invocation into a function call, and requires that we give the macro, which was originally untyped, a type signature.
If we were to only replace \verb|nonlinear|'s macro definition with a function definition at this point, however, we would introduce an undeclared reference error into the program, because the type of the argument \verb|axis| is defined \textit{after} the macro \verb|nonlinear| is defined.
Therefore, we must also move the \verb|AXIS| type's definition before the transformed definition of \verb|nonlinear|, or move \verb|nonlinear|'s transformed definition after the \verb|AXIS| type's definition.
The resulting code would look like this:
\begin{lstlisting}[style=CStyle]
typedef struct axis { ... } AXIS;
bool nonlinear(AXIS *axis) {
return axis->linked_to_primary != NULL && axis->link_udf->at != NULL;
}
AXIS *secondary;
if (nonlinear(secondary))
\end{lstlisting}

The penultimate portability level contains \textbf{argument-altering} code changes.
As their name suggests, argument-altering code changes affect a macro's arguments.
This means that we can make the macro more portable by turning it into a function call, while only making changes to the macro's definition and invocation.
This makes argument-altering code changes easier to reason about, and thus much more desirable than code changes in the first five levels.
For instance, consider the macro \verb|YYPOPSTACK| taken from \bash~\cite{bash-5.2-rc1}:

\begin{lstlisting}[style=CStyle]
#define YYPOPSTACK(N)   (yyvsp -= (N), yyssp -= (N))
yy_state_t *yyssp = ...;
YYSTYPE *yyvsp = ...;
YYPOPSTACK (1);|\label{line:invoke-yypopstack}|
\end{lstlisting}
In this example, the macro \verb|YYPOPSTACK| accepts a single argument \verb|N| of type \verb|int|.
When invoked on line~\ref{line:invoke-yypopstack}, it captures the variables \verb|yyvsp| and \verb|yyssp| from its caller's environment, and decrements them by \verb|N|.
Here is how we can use a argument-altering code change to turn \verb|YYPOPSTACK| into a function definition and its invocation into a function call:
\vspace{0.5em}
\begin{lstlisting}[style=CStyle]
void yypopstack(int N,
        yy_state_t **yyssp, YYSTYPE **yyvsp) {
    *yyvsp -= (N), *yyssp -= (N);
} 
yy_state_t *yyssp = ...;
YYSTYPE *yyvsp = ...;
yypopstack (1, &yyssp, &yyvsp);|\label{line:call-yypopstack}|
\end{lstlisting}
The first modification we make is to turn \verb|YYPOPSTACK|'s macro definition into a function definition.
This requires that we give the macro a type signature.
We give the function a \verb|void| return type because the original macro was only ever invoked for its side-effects.
We give the argument \verb|N| the type \verb|int| because whenever \verb|YYPOPSTACK| is invoked, a value of type \verb|int| is passed as the \verb|N| argument.
Next, because functions are lexically scoped and cannot capture variables from their callers' environments like macros can, we must add the arguments \verb|yyssp| and \verb|yyvsp| to the function's parameter list so that the caller can pass them to the function call at callsites.
Also, because functions follow a call-by-value calling convention, we have to turn these arguments into double pointers so that we can alter the values of \verb|yyssp| and \verb|yyvsp| in their caller's scope.
The last change we make is to pass the addresses of \verb|yyssp| and \verb|yyvsp| to the call to \verb|YYPOPSTACK| on line~\ref{line:call-yypopstack}

Finally, the most portable code changes are \textbf{\levelone} changes.
\levelone changes only modify the original code by replacing the invoked macro's definition with a function definition (or a variable or enum if the macro is object-like).
The macro's expected number and types of parameters do not change, so the macro's interface (i.e., the way the developer calls it) remains the same.
\levelone changes are especially convenient because they can turn all the original macro's invocations into function calls without requiring modifications to each invocation.
This is because macro invocations and function calls have the same syntax, so by replacing the invoked macro's definition with a function definition, the invocations immediately become function calls.
For example, the simple function-like macro \verb|gval| defined in \lua~\cite{lua} is invoked many times:
\begin{lstlisting}[style=CStyle]
typedef union Node {
    TValue i_val;
} Node;
#define gval(n)		(&(n)->i_val)
Node *n = ...;
lua_assert(isempty(gval(n)));
markvalue(g, gval(n));
setempty(gval(n));
\end{lstlisting}
In the above example, the macro \verb|gval| accepts a single argument \verb|n| of type \verb|Node *|.
It returns the address of \verb|n|'s \verb|i_val| field.
We can use a \levelone change to turn all of \verb|gval|'s invocations into function calls without needing to alter any of the invocations themselves:
\vspace{0.5em}
\begin{lstlisting}[style=CStyle]
TValue *gval(Node *n) {
    return (&(n)->i_val);
}
Node *n = ...;
lua_assert(isempty(gval(n)));
markvalue(g, gval(n));
setempty(gval(n));
\end{lstlisting}
Notice that the only modification we made was to replace \verb|gval|'s macro definition with a function definition.
Because macro invocations and function calls share the same syntax, all the invocations of \verb|gval| become function calls with no additional modifications necessary.
However, this also means that in order for an interface-equivalent transformation to result in correct code, all the invocations of the macro must expand to the same type and accept argument of the same respective types.
Otherwise, some calls of the transformed function may fail to typecheck.
If this happens, then the developer can either create a new suitably-typed function definition for each disinctly-typed invocation, or change the arguments and return types of all the macro's invocations to have the same type.

